Optimized Caching and Spectrum Partitioning for D2D enabled Cellular Systems with Clustered Devices

Caching at mobile devices and leveraging device- to-device (D2D) communication are two promising approaches to support massive content delivery over wireless networks. The analysis of cache-enabled wireless networks is usually carried out by assuming that devices are uniformly distributed, however, in social networks, mobile devices are intrinsically grouped into disjoint clusters. In this regards, this paper proposes a spatiotemporal mathematical model that tracks the service requests arrivals and account for the clustered devices geometry. Two kinds of devices are assumed, particularly, content clients and content providers. Content providers are assumed to have a surplus memory which is exploited to proactively cache contents from a known library, following a random probabilistic caching scheme. Content clients can retrieve a requested content from the nearest content provider in their proximity (cluster), or, as a last resort, the base station (BS). The developed spatiotemporal model is leveraged to formulate a joint optimization problem of the content caching and spectrum partitioning in order to minimize the average service delay. Due to the high complexity of the optimization problem, the caching and spectrum partitioning problems are decoupled and solved iteratively using the block coordinate descent (BCD) optimization technique. To this end, an optimal and suboptimal solutions are obtained for the bandwidth partitioning and probabilistic caching subproblems, respectively. Numerical results highlight the superiority of the proposed scheme over conventional caching schemes under equal and optimized bandwidth allocations. Particularly, it is shown that the average service delay is reduced by nearly 100% and 350%, compared to the Zipf and uniform caching schemes under equal bandwidth allocations, respectively.

==> Optimized Caching and Spectrum Partitioning for D2D enabled Cellular Systems with Clustered Devices/acronyms.tex <==

\acro{OFDM}{orthogonal frequency-division multiplexing}
\acro{OFDMA}{orthogonal frequency-division multiple access}
\acro{MNO}{mobile network operator}
\acro{RA}{resource allocation}
\acro{SC-FDMA}{single carrier frequency division multiple access}
\acro{CR}{cognitive radio}
\acro{RFIC}{radio frequency integrated circuit} 
\acro{SDR}{software defined radio}
\acro{SDN}{software defined networking}
\acro{su}{secondary user}
% \acro{SU}{Internet of Things}
\acro{QoS}{quality-of-service}
\acro{USRP}{universal software radio peripheral}
\acro{GSM}{Global System for Mobile Communications}
\acro{TDMA}{time-division multiple access}
\acro{FDMA}{frequency-division multiple access}
\acro{GPRS}{General Packet Radio Service}
\acro{MSC}{Mobile Switching Centre}
\acro{BSC}{Base Station Controller}
\acro{UMTS}{Universal Mobile Telecommunications System}
\acro{WCDMA}{wide-band code division multiple access}
\acro{CDMA}{code division multiple access}
\acro{LTE}{Long Term Evolution}
\acro{PAPR}{peak-to-average power rating}
\acro{HetNet}{heterogeneous networks}
\acro{PHY}{physical layer}
\acro{MAC}{medium access control}
\acro{AMC}{adaptive modulation and coding}
\acro{MIMO}{multiple-input multiple-output}
\acro{M-MIMO}{massive MIMO}
\acro{RAT}{radio access technology}
\acro{VNI}{visual networking index}
\acro{RB}{resource block}
\acro{UE}{user equipment}
\acro{CQI}{channel quality indicator}
\acro{HD}{half duplex}
\acro{IBFD}{in-band full duplex}
\acro{SIC}{self-interference cancellation}
\acro{SI}{self-interference}
\acro{BS}{base station}
\acro{FBMC}{filter bank multi-carrier}
\acro{UFMC}{universal filtered multi-carrier}
\acro{SCM}{single carrier modulation}
\acro{isi}{inter-symbol interference}
\acro{FTN}{faster-than-nyquist}
\acro{M2M}{machine-to-machine}
\acro{MTC}{machine type communication}
\acro{mmWave}{millimeter wave}
\acro{BF}{beamforming}
\acro{LoS}{line-of-sight}
\acro{NLoS}{non-line-of-sight}
\acro{CAPEX}{capital expenditure}
\acro{OPEX}{operational expenditure}
\acro{ICT}{information and communications technology}
\acro{SP}{service providers}
\acro{InP}{infrastructure providers}
\acro{MVNP}{mobile virtual network provider}
\acro{MVNO}{mobile virtual network operator}
\acro{NFV}{network function virtualization}
\acro{VNF}{virtual network functions}
\acro{C-RAN}{cloud radio access network}
\acro{RAN}{radio access network}
\acro{BBU}{baseband unit}
\acro{RRH}{remote radio head}
\acro{TDD}{time-division duplexing}
\acro{FDD}{frequency-division duplexing}
\acro{GFDM}{generalized frequency division multiplexing}
\acro{CSI}{channel state information}
\acro{FFT}{fast Fourier transform}
\acro{IFFT}{inverse FFT}
\acro{CFO}{carrier frequency offset}
\acro{CoMP}{coordinated multipoint}
\acro{D2D}{device-to-device}
\acro{OOB}{out-of-band}
\acro{TTI}{transmission time interval}
% \acro{RAT}{radio access technology}
%\acrodefplural{rat}[RATs]{radio access technologies}
\acro{DUE}{D2D user equipment}
\acro{DAS}{distributed antenna system}
\acro{ICIC}{inter-cell interference coordination}
\acro{ICI}{inter-cell interference}
\acro{ISI}{inter-symbol interference}
\acro{CP}{cyclic prefix}
\acro{PDF}{probability distribution function}
\acro{KPI}{key performance indicator}
%\acro{CoMP}{coordinated multipoint}
\acro{SBS}{small base station}
\acro{MBS}{macro base station}
\acro{SCN}{small cell network}
\acro{FIFO}{first in first out}
\acro{VCC}{virtual cache center}
\acro{UAV}{unmanned aerial vehicles}
\acro{MPSQ}{multiclass processor sharing queue} 
\acro{EE}{energy efficiency}
\acro{SIR}{signal-to-interference ratio}
\acro{SINR}{signal-to-noise-plus-interference ratio}
\acro{PPP}{Poisson point process}
\acro{PCP}{Poisson cluster process}
% \acro{BS}{base station}
\acro{HCP}{hard-core placement} 
\acro{TCP}{Thomas cluster process }
\acro{CPF}{caching popular files}
\acro{GCA}{greedy caching algorithm }
\acro{RC}{random caching }
\acro{PC}{probabilistic caching}
% \acro{ICIC}{intercell interference coordination}
\acro{5G}{fifth generation}
\acro{MEC}{mobile edge computing}
\acro{AP}{access point}
% \acro{SDN}{software-defined networking}
% \acro{NFV}{network functions virtualization}
\acro{VoD}{video-on-demand}
\acro{EPC}{evolved packet core}
\acro{QoE}{quality-of-experience}
\acro{CDN}{content delivery networks}
% \acro{BBU}{baseband signal processing uni}
\acro{F-RAN}{fog-radio access network}
\acro{AR}{augmented reality}
\acro{VR}{virtual reality}
% \acro{HetNets}[HetNets]{heterogeneous networks}
\acro{4C}{computing, caching, communication, and control}
\acro{ABR}{Adaptive BitRate}
\acro{ILP}{Integer Linear Program}
\acro{MILP}{Mixed Integer Linear Program}
\acro{MINLP}{Mixed Integer Non-Linear Program}
\acro{BC}{broadcast channel}
\acro{MDS}{maximum distance separable}
\acro{RS}{Reed-Solomon}
\acro{NC}{network coding}
% \acro{SIC}{successive interference cancellation}
\acro{MSR}{minimum storage regenerating}
\acro{Coop-MIMO}{cooperative \ac{mimo}}
\acro{UDN}{ultra-dense networks}
\acro{ETSI}{European Telecommunications Standards Institute}
\acro{MCP}{Matern cluster process}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \acro{D2D}{device-to-device}
% \acro{SIR}{signal-to-interference-ratio}
% \acro{SINR}{signal-to-interference-plus-noise-ratio}
% \acro{PCP}{Poisson cluster process}
%\acro{CoMP}{coordinated multi-point}
% \acro{BS}{base station} 
\acro{MD-CoMP}{macrodiversity CoMP transmission}
% \acro{MAC}{medium-access-control}
\acro{JT-CoMP}{joint transmission CoMP}
\acro{CoMP-JT}{coordinated multipoint joint transmission}
% \acro{SBS}{small base station}
\acro{MDSD}{multiple devices to the single device}
% \acro{MDS}{maximum distance separable}
% \acro{SCN}{small cell network}
% \acro{PPP}{Poisson point process}
% \acro{TCP}{Thomas cluster process}
% \acro{CSI}{channel state information}
% \acro{PDF}{probability distribution function}
\acro{PMF}{probability mass function}
\acro{RV}{random variable}
\acro{i.i.d.}{independently and identically distributed}
\acro{MBMS}{multimedia broadcasting multicasting service}
% \acro{EE}{energy efficiency}
% \acro{HCP}{hard-core placement}
\acro{CCDF}{complementary cumulative distribution function}
\acro{CDF}{cumulative distribution function}
% \acro{PC}{probabilistic caching}
% \acro{RC}{random uniform caching}
% \acro{CPF}{caching popular files} 
\acro{PGFL}{probability generating functional}
\acro{KKT}{Karush-Kuhn-Tucker}
\acro{PGF}{point generating function}
\acro{BPP}{binomial point process}
\acro{3GPP}{3rd Generation Partnership Project}
% \acro{UAV}{unmanned aerial vehicle}
\acro{FAA}{Federal Aviation Administration}
\acro{UAS}{unmanned aircraft systems}
% \acro{AP}{access point}
% \acro{GSM}{Global System for Mobile Communications}
% \acro{LTE}{long term evolution}
\acro{IoT}{Internet-of-things}
% \acro{UE}{user equipment}
\acro{CNPC}{control and non-payload communication}
\acro{FHD}{full high definition}
%\acro{NLoS}{non-line-of-sight}
%\acro{LoS}{line-of-sight}
% \acro{5G}{fifth-generation}
\acro{MGF}{moment generating function}
\acro{3D}{three-dimensional}
\acro{2D}{two-dimensional}
\acro{1D}{one-dimensional}
% \acro{MIMO}{multiple-input multiple-output}
\acro{CB}{conjugate beamforming}
\acro{AU}{aerial user}
\acro{GU}{ground user}
\acro{CLT}{central limit theorem}
\acro{SE}{spectral efficiency}
\acro{MRT}{maximum ratio transmission}
\acro{ZFBF}{zero-forcing beamforming}
% \acro{QoS}{quality-of-service}
\acro{GBS}{ground base station}
% \acro{F-RAN}{fog-radio access network}
% \acro{RAN}{radio access network}
% \acro{RRH}{remote radio head}
% \acro{mmWave}{millimeter wave}
\acro{C&C}{command and control}
\acro{ASE}{area spectral efficiency}
\acro{RWP}{random waypoint}
\acro{AGL}{above ground level}
\acro{w.r.t.}{with respect to}
\acro{GTA}{ground-to-air}
% \acro{user equipment}{UE}
\acro{AUE}{aerial user equipment}
\acro{GUE}{ground user equipment}
\acro{UB}{upper bound}
\acro{LB}{lower bound}
\acro{ABS}{aerial base station}
\acro{UAV-UE}{UAV-\ac{UE}}
\acro{SCDP}{successful content delivery probability}
\acro{HARP}{highest average received power}
\acro{ULA}{uniform linear array}
\acro{GPP}{Gaussian Poisson process}
\acro{NSD}{nearest serving device}
\acro{NCP}{nearest content provider}
\acro{RSD}{randomly serving device}
\acro{RSCP}{randomly-selected content provider}
\acro{BCD}{block coordinate descent}
\acro{NOMA}{non-orthogonal multiple access}
\acro{MPC}{most popular content}
\acro{LPC}{least popular content}
\acro{AI}{artificial intelligence}
\acro{ML}{machine learning}
\acro{TPP}{temporal point process}
\acro{PP}{point process}
\acro{DPP}{Determinantal point process}
\acro{DPPL}{DPP-based learning}
\acro{DRL}{deep reinforcement learning}
\acro{RL}{reinforcement learning}
\acro{RNN}{recurrent neural network}
\acro{RMTPP}{recurrent marked TPP}
\acro{NR}{New Radio}
\acro{HO}{handover}
\acro{RLF}{radio link failure}
\acro{RSRP}{reference signal received power}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}











==> Optimized Caching and Spectrum Partitioning for D2D enabled Cellular Systems with Clustered Devices/mypackage.tex <==


\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{url}
\usepackage{ifthen}
\usepackage{cite}
\usepackage[cmex10]{amsmath} % Use the [cmex10] option to ensure complicance
\usepackage{stackengine}
\usepackage{gensymb}
\usepackage{graphics}
\usepackage{mypackage}
\usepackage{mathrsfs}

%% Ramy &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&
\usepackage{mathtools}
\usepackage{tabu}
\usepackage{float}
\usepackage{physics}
\usepackage{siunitx}
\usepackage{multicol}
\usepackage{amssymb}
\usepackage[nomain,acronym,shortcuts]{glossaries}

\usepackage{etoolbox}

==> Optimized Caching and Spectrum Partitioning for D2D enabled Cellular Systems with Clustered Devices/newcommands.tex <==

\newcommand{\sinr}{\mathrm{SINR}}
\newcommand{\sir}{\mathrm{SIR}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\Eb}{\mathbb{E}}
\newcommand{\Rb}{\mathbb{R}}
\newcommand{\Rs}{\mathbb{R}^2}
\newcommand{\Rp}{\mathbb{R}^+}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\e}{\mathcal{E}} 
\newcommand{\eav}{\mathcal{E_{av}}} 
\newcommand{\pc}{\mathrm{P_c}}
\newcommand{\pcd}{\mathrm{P_{c_d}}}
\newcommand{\pcb}{\mathrm{P_{c_b}}}
\newcommand{\besselI}[1]{\mbox{I$_0$}(#1)}


\def\delequal{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptscriptstyle\Delta}}}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

 \makeglossaries
\newcommand*{\acro}[3][]{\newacronym[#1]{#2}{#2}{#3}}


\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\theoremstyle{approximation}
\newtheorem{approximation}{Approximation}
%\newtheorem{definition}{Definition}

\newcommand{\Chi}{\mathrm{X}}
\newcommand{\Alpha}{\mathrm{A}}


\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\black}{\textcolor{black}}
\newcommand{\green}{\textcolor{green}}
\newcommand{\magenta}{\textcolor{magenta}}

\newcommand{\Eq}[1]{(\ref{eq:#1})}
\newcommand{\App}[1]{Appendix~\ref{app:#1}}
\newcommand{\Fig}[1]{Fig.~\ref{fig:#1}}

\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\R}{\mathbb{R}}
\DeclareMathOperator*{\N}{\mathcal{N}}
\DeclareMathOperator*{\U}{\mathcal{U}}
\DeclareMathOperator*{\CN}{\mathcal{CN}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Joint Cache and Delay CH(3)
\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CoMP Ch(4)
\newcounter{MYtempeqncnt}
\def\delequal{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Baza Ismail for references 
\let\mybibitem\bibitem
\renewcommand{\bibitem}[1]{%
  \ifstrequal{#1}{nature}
    {\color{blue}\mybibitem{#1}}
    {\color{black}\mybibitem{#1}}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% IEEE CL
%\def\delequal{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptscriptstyle\Delta}}}}





